PAQ: 65 Million Probably-Asked Questions and What You Can Do With Them

Open-domain Question Answering models which directly leverage question-answer (QA) pairs, such as closed-book QA (CBQA) models and QA-pair retrievers, show promise in terms of speed and memory compared to conventional models which retrieve and read from text corpora. QA-pair retrievers also offer interpretable answers, a high degree of control, and are trivial to update at test time with new knowledge. However, these models lack the accuracy of retrieve-and-read systems, as substantially less knowledge is covered by the available QA-pairs relative to text corpora like Wikipedia. To facilitate improved QA-pair models, we introduce Probably Asked Questions (PAQ), a very large resource of 65M automatically-generated QA-pairs. We introduce a new QA-pair retriever, RePAQ, to complement PAQ. We find that PAQ preempts and caches test questions, enabling RePAQ to match the accuracy of recent retrieve-and-read models, whilst being significantly faster. Using PAQ, we train CBQA models which outperform comparable baselines by 5%, but trail RePAQ by over 15%, indicating the effectiveness of explicit retrieval. RePAQ can be configured for size (under 500MB) or speed (over 1K questions per second) whilst retaining high accuracy. Lastly, we demonstrate RePAQ's strength at selective QA, abstaining from answering when it is likely to be incorrect. This enables RePAQ to ``back-off" to a more expensive state-of-the-art model, leading to a combined system which is both more accurate and 2x faster than the state-of-the-art model alone.

==> background_sr.tex <==
\section{Open-Domain Question Answering}

ODQA is the task of answering factoid questions $q$ expressed in natural language with answers $a=h(q)$ from an open set of domains.
%
A typical question might be "when was the last year astronauts landed on the moon?", with the target answer answer "1972".
%
We assume there is a distribution $P(q,a)=P(q)P(a|q)$ of questions and their answers.
%
%
However, in general we cannot directly access $P$, and instead rely on an empirical sample of QA-pairs $\mathcal{K}$ drawn from $P$, and train $h$ to minimise the empirical loss on $\mathcal{K}$.
%
Usually this sample will only capture a small fraction of the questions that are likely to be asked in practice.
%
The standard approach in ODQA is to estimate a \emph{conditional} $p(a|q)$.
%
In this paper, our principle goal is to estimate a joint distribution $p(q,a)$ that approximates $P(q,a)$ in order to generate a much larger empirical sample that has greater coverage of the questions we expect people to ask.

* Our hypothesis is that this sample, PAQ, is important for training/developing more accurate, efficient and calibrated ODQA models of today's architectures (closed book, question retrieval, open book), as we show the results section.  
 

% * ODQA is the task of answering (factoid) questions $q$ with answers $a=h(q)$. For example, ... some example question and answer. 
% * We assume there is a distribution $P(q,a)=P(q)P(a|q)$ of questions and their answers. This distribution captures both how likely a particular question will be asked via $P(q)$, and what the correct answers are via $P(a|q)$. For example, in a web search setting, P("When is the next episode of ...") is higher than P(...some other more obscure question), and something something about P(June 12|When is the next episode..) is bigger than ...
% * A good answer function $h(a)$ will minimise the \emph{expected} loss over $P$ with respect to some loss function (e.g. exact match of the answer string). However, in general we don't have access to $P$ but only to an empirical sample $D=...$ and hence we train $h$ to minimise the \emph{empirical} loss on that sample as an approximation. Usually this sample will only capture a small fraction of the questions that are likely to be asked in practice
% * The standard approach in ODQA is to estimate a \emph{conditional} $p(a|q)$, usually with access to a background corpus of knowledge (but not necessarily). $h(q)$ is then simply choosing the argmax... Previous work has found that in this approach either implicitly (closed book and open book) or explicitly (question retrieval), current architectures primarily rely on the empirical training sample for answering questions anyway and show little signs of generalisation.
% * Motivated by this observation, In this paper, our principle goal is to estimate a \emph{joint} distribution $p(q,a)$ that approximates the ``real'' $P(q,a)$ in order to generate an approximate empirical sample (aka PAQ) that has much larger coverage of the questions we expect people to ask.
% * Our hypothesis is that this sample, PAQ, is critical for training/developing more accurate, efficient and calibrated ODQA models of today's architectures (closed book, question retrieval, open book), as we show the results section.  


